Predictably Missing Satellites: Subhalo Abundance in Milky Way-like Halos

On small scales there have been a number of claims of discrepancies between the standard Cold Dark Matter (CDM) model and observations. The 'missing satellites problem' infamously describes the overabundance of subhalos from CDM simulations compared to the number of satellites observed in the Milky Way. A variety of solutions to this discrepancy have been proposed; however, the impact of the specific properties of the Milky Way halo relative to the typical halo of its mass have yet to be explored. Motivated by recent studies that identified ways in which the Milky Way is atypical (e.g., Licquia et al. 2015), we investigate how the properties of dark matter halos with mass comparable to our Galaxy's --- including concentration, spin, shape, and scale factor of the last major merger --- correlate with the subhalo abundance. Using zoom-in simulations of Milky Way-like halos, we build two models of subhalo abundance as functions of host halo properties and conclude that the Milky Way should be expected to have 22%-44% fewer subhalos with low maximum rotation velocities ($V_{\rm max}^{\rm sat} \sim 10$kms$^{-1}$) at the 95% confidence level and up to 72% fewer than average subhalos with high rotation velocities ($V_{\rm max}^{\rm sat} \gtrsim 30$kms$^{-1}$, comparable to the Magellanic Clouds) than would be expected for a typical halo of the Milky Way's mass. Concentration is the most informative single parameter for predicting subhalo abundance. Our results imply that models tuned to explain the missing satellites problem assuming typical subhalo abundances for our Galaxy will be over-correcting.

==> hyperlink-year-only-natbib-patch.tex <==
% found on https://tex.stackexchange.com/questions/23227/how-to-hyperlink-only-the-year-part-when-using-natbib-and-hyperref

\RequirePackage{hyperref}
\RequirePackage{natbib}
\RequirePackage{etoolbox}

\makeatletter

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother

